Magic3DSketch: Create Colorful 3D Models From Sketch-Based 3D Modeling Guided by Text and Language-Image Pre-Training

The requirement for 3D content is growing as AR/VR application emerges. At the same time, 3D modelling is only available for skillful experts, because traditional methods like Computer-Aided Design (CAD) are often too labor-intensive and skill-demanding, making it challenging for novice users. Our proposed method, Magic3DSketch, employs a novel technique that encodes sketches to predict a 3D mesh, guided by text descriptions and leveraging external prior knowledge obtained through text and language-image pre-training. The integration of language-image pre-trained neural networks complements the sparse and ambiguous nature of single-view sketch inputs. Our method is also more useful and offers higher degree of controllability compared to existing text-to-3D approaches, according to our user study. Moreover, Magic3DSketch achieves state-of-the-art performance in both synthetic and real dataset with the capability of producing more detailed structures and realistic shapes with the help of text input. Users are also more satisfied with models obtained by Magic3DSketch according to our user study. Additionally, we are also the first, to our knowledge, add color based on text description to the sketch-derived shapes. By combining sketches and text guidance with the help of language-image pretrained models, our Magic3DSketch can allow novice users to create custom 3D models with minimal effort and maximum creative freedom, with the potential to revolutionize future 3D modeling pipelines.

==> table/table1.tex <==
% %% table 1
% \begin{table*}[ht]
% \begin{center}
% \caption{The quantitative evaluation of ShapeNet-Synthetic dataset}
% \scalebox{1}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{8}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow)$} \\
% \hline
%  & car & sofa & airplane & bench & display & chair & table \\
% \hline
% Retrieval & 0.667 & 0.483 & 0.513 & 0.38  & 0.385 & 0.346 & 0.311 \\
% \hline
% Auto-Encoder & 0.769 & 0.613 & 0.576 & 0.467 & 0.541 & 0.496 & 0.512 \\
% \hline
% Sketch2Model (GT Pos)  & 0.751 & 0.622 & 0.624 & 0.481 & 0.604 & 0.522 & 0.478 \\
% Sketch2Model (Pred Pos) & 0.746 & 0.620 & 0.618 & 0.477 & 0.550 & 0.515 & 0.470 \\
% \hline
% \textbf{Ours (GT Pos)} & \textbf{0.796} & \textbf{0.651} & \textbf{0.644} & \textbf{0.500} & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} \\
% \textbf{Ours (Pred Pos)} & 0.793 & 0.649 & 0.641 & \textbf{0.500} & 0.583 & 0.541 & 0.504 \\
% \hline
%  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
% \hline
% Retrieval & 0.622 & 0.518 & 0.468 & 0.422 & 0.325 & 0.475 & 0.455 \\
% \hline
% Auto-Encoder & 0.706 & 0.663 & 0.629 & 0.556 & 0.431 & 0.605 & 0.582 \\
% \hline
% Sketch2Model (GT Pos) & 0.719 & 0.701 & 0.641 & 0.586 & 0.472 & 0.612 & 0.601 \\
% Sketch2Model (Pred Pos) & 0.673 & 0.667 & 0.624 & 0.569 & 0.463 & 0.606 & 0.584 \\
% \hline
% \textbf{Ours (GT Pos)} & \textbf{0.738} & \textbf{0.705} & \textbf{0.651} & \textbf{0.595} & \textbf{0.469} & \textbf{0.619} & \textbf{0.618} \\ 
% \textbf{Ours (Pred Pos)} & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & \textbf{0.619} & 0.604 \\
% \hline
% \end{tabular}}
% \end{center}

% \label{table:table2}

% \end{table*}


%% table 1  -------
% \begin{table*}[ht]
% \begin{center}
% \caption{The quantitative evaluation of ShapeNet-Synthetic dataset}
% \scalebox{0.88}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{8}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow$)} \\
% \hline
%  & car & sofa & airplane & bench & display & chair & table \\
% \hline
% Retrieval & 0.667 & 0.483 & 0.513 & 0.38  & 0.385 & 0.346 & 0.311 \\
% \hline
% Auto-Encoder & 0.769 & 0.613 & 0.576 & 0.467 & 0.541 & 0.496 & 0.512 \\
% \hline
% Sketch2Model (GT Pos)  & 0.751 $\pm$ 0.119 & 0.622 $\pm$ 0.163 & 0.624 $\pm$ 0.144 & 0.481 $\pm$ 0.149 & 0.604 $\pm$  & 0.522 $\pm$ 0.154 & 0.478 $\pm$ 0.181 \\
% Sketch2Model (Pred Pos) & 0.746 $\pm$ 0.124 & 0.620 $\pm$ 0.161 & 0.618 $\pm$ 0.149  & 0.477 $\pm$ 0.153 & 0.550 $\pm$ & 0.515 $\pm$ 0.155 & 0.470 $\pm$ 0.181 \\
% \hline
% \textbf{Ours (GT Pos)} & \textbf{0.796 $\pm$} & \textbf{0.651 $\pm$} & \textbf{0.644 $\pm$} & \textbf{0.500 $\pm$} & \textbf{0.612 $\pm$}	& \textbf{0.544 $\pm$ & \textbf{0.518 $\pm$} \\
% \textbf{Ours (Pred Pos)} & 0.793 $\pm$ & 0.649 $\pm$ & 0.641 $\pm$ & \textbf{0.500} $\pm$ & 0.583 $\pm$ & 0.541 $\pm$ & 0.504 $  \pm $\\
% \hline
%  & telephone & cabinet & loudspeaker & watercraft & lamp & rifle & mean \\
% \hline
% Retrieval & 0.622 & 0.518 & 0.468 & 0.422 & 0.325 & 0.475 & 0.455\\
% \hline
% Auto-Encoder & 0.706 & 0.663 & 0.629 & 0.556 & 0.431 & 0.605 & 0.582 \\
% \hline
% Sketch2Model (GT Pos)  & 0.719 $\pm$ 0.207 & 0.701 $\pm 0.209 $ & 0.641 $\pm$ 0.208 & 0.586 $\pm$ 0.161 & 0.472 $\pm$ 0.208 & 0.612 $\pm$ 0.170 & 0.601 $\pm$\\
% Sketch2Model (Pred Pos) & 0.673 $\pm$ 0.216 & 0.667$\pm 0.220 $ & 0.624 $\pm$ 0.216 & 0.569 $\pm$ 0.168 & 0.463 $\pm$ 0.209 & 0.606 $\pm$ 0.172 & 0.584 $\pm$ \\
% \hline
% \textbf{Ours (GT Pos)} & \textbf{0.738 $\pm$} & \textbf{0.705 $\pm$} & \textbf{0.651 $\pm$} & \textbf{0.595 $\pm$} & \textbf{0.469 $\pm$} & \textbf{0.619 $\pm$} & \textbf{0.618 $\pm$}  \\
% \textbf{Ours (Pred Pos)} & 0.680 $\pm$ & 0.683 $\pm$ & 0.623 $\pm$ & 0.580 $\pm$ & 0.465 $\pm$ & \textbf{0.619 $\pm$} & 0.604 $\pm$ \\
% \hline
% \end{tabular}}
% \end{center}
% \label{table:table2}
% \end{table*}


\begin{table*}[ht]
\centering
\caption{The quantitative evaluation of ShapeNet-Synthetic dataset}
\scalebox{0.88}{  % 调整表格大小适合页面宽度
\begin{tabular}{|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{8}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow$)} \\
\hline
 & car & sofa & airplane & bench & display & chair & table \\
\hline
Retrieval & 0.667 & 0.483 & 0.513 & 0.38  & 0.385 & 0.346 & 0.311 \\
\hline
Auto-Encoder & 0.769 & 0.613 & 0.576 & 0.467 & 0.541 & 0.496 & 0.512 \\
\hline
Sketch2Model (GT Pos)  & 0.751 $\pm$ 0.119 & 0.622 $\pm$ 0.163 & 0.624 $\pm$ 0.144 & 0.481 $\pm$ 0.149 & 0.604 $\pm$ 0.135 & 0.522 $\pm$ 0.154 & 0.478 $\pm$ 0.181 \\
Sketch2Model (Pred Pos) & 0.746 $\pm$ 0.124 & 0.620 $\pm$ 0.161 & 0.618 $\pm$ 0.149  & 0.477 $\pm$ 0.153 & 0.550 $\pm$ 0.134 & 0.515 $\pm$ 0.155 & 0.470 $\pm$ 0.181 \\
\hline
\textbf{Ours (GT Pos)} & \textbf{0.796 $\pm$ 0.132} & \textbf{0.651 $\pm$ 0.159} & \textbf{0.644 $\pm$ 0.149} & \textbf{0.500 $\pm$ 0.153} & \textbf{0.612 $\pm$ 0.182}	& \textbf{0.544 $\pm$ 0.152} & \textbf{0.518 $\pm$ 0.187} \\
\textbf{Ours (Pred Pos)} & 0.793 $\pm$ 0.133 & 0.649 $\pm$ 0.158 & 0.641 $\pm$ 0.153 & \textbf{0.500} $\pm$ 0.153 & 0.583 $\pm$ 0.195 & 0.541 $\pm$ 0.152 & 0.504 $\pm$ 0.190 \\
\hline
 & telephone & cabinet & loudspeaker & watercraft & lamp & rifle & mean \\
\hline
Retrieval & 0.622 & 0.518 & 0.468 & 0.422 & 0.325 & 0.475 & 0.455\\
\hline
Auto-Encoder & 0.706 & 0.663 & 0.629 & 0.556 & 0.431 & 0.605 & 0.582 \\
\hline
Sketch2Model (GT Pos)  & 0.719 $\pm$ 0.207 & 0.701 $\pm$ 0.209 & 0.641 $\pm$ 0.208 & 0.586 $\pm$ 0.161 & 0.472 $\pm$ 0.208 & 0.612 $\pm$ 0.170 & 0.601\\
Sketch2Model (Pred Pos) & 0.673 $\pm$ 0.216 & 0.667 $\pm$ 0.220 & 0.624 $\pm$ 0.216 & 0.569 $\pm$ 0.168 & 0.463 $\pm$ 0.209 & 0.606 $\pm$ 0.172 & 0.584 \\
\hline
\textbf{Ours (GT Pos)} & \textbf{0.738 $\pm$ 0.201} & \textbf{0.705 $\pm$ 0.209} & \textbf{0.651 $\pm$ 0.206} & \textbf{0.595 $\pm$ 0.158} & \textbf{0.469 $\pm$ 0.207} & \textbf{0.619 $\pm$ 0.174} & \textbf{0.618}  \\
\textbf{Ours (Pred Pos)} & 0.680 $\pm$ 0.232 & 0.683 $\pm$ 0.216 & 0.623 $\pm$ 0.212 & 0.580 $\pm$ 0.164 & 0.465 $\pm$ 0.209 & \textbf{0.619 $\pm$ 0.174} & 0.604\\
\hline
\end{tabular}
}
\end{table*}




% Please add the following required packages to your document preamble:
% \usepackage[table,xcdraw]{xcolor}
% If you use beamer only pass "xcolor=table" option, i.e. \documentclass[xcolor=table]{beamer}


%% table 2

% \begin{table*}[ht]
% \begin{center}
% \caption{The quantitative evaluation of ShapeNet-Sketch dataset}
% \scalebox{0.84}{

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% & {\color[HTML]{333333} Cabinet} & {\color[HTML]{333333} Bench} & {\color[HTML]{333333} Display} & {\color[HTML]{333333} Loudspeaker} & {\color[HTML]{333333} Telephone} & {\color[HTML]{333333} Rifile} & {\color[HTML]{333333} Watercraft} & {\color[HTML]{333333} Lamp} & {\color[HTML]{333333} Airplane} & {\color[HTML]{333333} Sofa} & {\color[HTML]{333333} Table} & {\color[HTML]{333333} Chair} & {\color[HTML]{333333} Car} & mean           \\ \hline
% sketch2model                & \textbf{0.568}                 & 0.366                        & \textbf{0.479}                 & \textbf{0.544}                     & 0.554                            & 0.534                         & 0.466                             & 0.338                       & 0.487                           & 0.534                       & 0.357                        & \textbf{0.393}               & 0.659                      & 0.483          \\ \hline
% deep3dsketch+               & 0.553                          & 0.368                        & 0.463                          & 0.514                              & \textbf{0.576}                   & 0.543                         & 0.467                             & \textbf{0.347}              & \textbf{0.490}                  & \textbf{0.534}              & 0.370                        & 0.382                        & 0.675                      & 0.483          \\ \hline
% { Ours} & 0.551                          & \textbf{0.374}               & 0.456                          & 0.503                              & 0.557                            & \textbf{0.553}                & \textbf{0.473}                    & 0.339                       & 0.489                           & 0.533                       & \textbf{0.381}               & 0.389                        & \textbf{0.695}             & \textbf{0.484} \\ \hline
% \end{tabular}}

% \end{center}

% \label{table:table3}

% \end{table*}


%% table 1
% \begin{table*}[ht]
% \begin{center}
% \caption{The quantitative evaluation of ShapeNet-Synthetic dataset}
% \scalebox{1}{
% \begin{tabular}{|c |c |c |c |c |c |c |c}
% \hline
% \multicolumn{8}{c}{Shapenet-synthetic (Voxel Iou $\uparrow)$} \\
%  & car & sofa & airplane & bench & display & chair & table \\
% \hline
% Retrieval & 0.667 & 0.483 & 0.513 & 0.38  & 0.385 & 0.346 & 0.311 \\

% Auto-Encoder & 0.769 & 0.613 & 0.576 & 0.467 & 0.541 & 0.496 & 0.512 \\

% Sketch2Model (GT Pos)  & 0.751 & 0.622 & 0.624 & 0.481 & 0.604 & 0.522 & 0.478 \\
% Sketch2Model (Pred Pos) & 0.746 & 0.620 & 0.618 & 0.477 & 0.550 & 0.515 & 0.470 \\

% \textbf{Ours (GT Pos)} & \textbf{0.796} & \textbf{0.651} & \textbf{0.644} & \textbf{0.500} & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} \\
% \textbf{Ours (Pred Pos)} & 0.793 & 0.649 & 0.641 & \textbf{0.500} & 0.583 & 0.541 & 0.504 \\
% \hline
%  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
% \hline
% Retrieval & 0.622 & 0.518 & 0.468 & 0.422 & 0.325 & 0.475 & 0.455 \\

% Auto-Encoder & 0.706 & 0.663 & 0.629 & 0.556 & 0.431 & 0.605 & 0.582 \\

% Sketch2Model (GT Pos) & 0.719 & 0.701 & 0.641 & 0.586 & 0.472 & 0.612 & 0.601 \\
% Sketch2Model (Pred Pos) & 0.673 & 0.667 & 0.624 & 0.569 & 0.463 & 0.606 & 0.584 \\

% \textbf{Ours (GT Pos)} & \textbf{0.738} & \textbf{0.705} & \textbf{0.651} & \textbf{0.595} & \textbf{0.469} & \textbf{0.619} & \textbf{0.618} \\ 
% \textbf{Ours (Pred Pos)} & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & \textbf{0.619} & 0.604 \\
% \hline
% \end{tabular}}
% \end{center}

% \label{table:table2}

% \end{table*}


==> table/table2.tex <==

%% table 2

\begin{table*}[ht]
\begin{center}
\caption{The quantitative evaluation of ShapeNet-Sketch dataset}
\scalebox{0.84}{

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\hline
\multicolumn{15}{|c|}{Shapenet-sketch (Voxel IoU $\uparrow$)} \\
\hline
 & car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean\\
\hline
Retrieval & 0.626 & 0.431 & 0.411 & 0.219 & 0.338 & 0.238 & 0.232 & 0.536 & 0.431 & 0.365 & 0.369 & 0.223 & 0.413 & 0.370\\
\hline
Auto-Encoder & 0.648 & 0.534 & 0.469 & 0.347 & 0.472 & 0.361 & 0.359 & 0.537 & 0.534 & 0.533 & 0.456 & 0.328 & 0.541 & 0.372 \\
\hline
Sketch2Model (GT Pos)  & 0.659 & 0.534 & 0.487 & 0.366 & 0.479 & 0.393 & 0.357 & 0.554 & \textbf{0.568} & 0.526 & 0.450 & \textbf{0.338} & 0.534 & 0.483 \\
Sketch2Model (Pred Pos) & 0.649 & 0.528 & 0.479 & 0.357 & 0.435 & 0.383 & 0.361 & 0.551 & 0.547 & 0.544 & 0.466 & 0.336 & 0.510 & 0.470\\
\hline
Sketch2Model + DA (GT Pos) & 0.679  & \textbf{0.548} & \textbf{0.526} & \textbf{0.367} & - & \textbf{0.398} & 0.357 & - & - & - & - & - & 0.535 & 0.489\\
Sketch2Model + DA (Pred Pos) & 0.659 & 0.533 & 0.515 & 0.362 & - & 0.385 & 0.360  & - & - & - & - & - & 0.511 & 0.475 \\
\hline
\textbf{Ours (GT Pos)} & 0.695 & 0.528 & 0.502 & 0.364 & \textbf{0.493} & 0.389 & 0.370 & \textbf{0.574} & 0.563 & \textbf{0.538} & \textbf{0.477} & 0.334 & 0.535 & 0.489 \\
\textbf{Ours (Pred Pos)} & 0.683 & 0.523 & 0.502 & 0.364 & 0.493 & 0.389 & \textbf{0.370} & 0.527 & 0.549 & 0.509 & 0.468 & 0.331 & 0.535 & 0.476 \\
\hline
\textbf{Ours + DA (GT Pos)}   & \textbf{0.699} & 0.538 & 0.517 & 0.362 & - & 0.390 & 0.360 & - & - & - & - & - & \textbf{0.545} & \textbf{0.491} \\
\textbf{Ours + DA (Pred Pos)} & 0.692 & 0.532 & 0.515 & 0.360 & - & 0.382 & 0.346  & - &  & - & - & - & \textbf{0.545} & 0.477\\
\hline

\end{tabular}}
\end{center}

\label{table:table3}

\end{table*}

==> table/table3.tex <==


%% table 3
\begin{table*}[h]
\caption{{The quantitative evaluation of ablation study.} }
\begin{center}
\scalebox{1}{
\begin{tabular}{|c c | c| c| c| c| c| c| c |}
\hline
\multicolumn{9}{|c|}{Ablation Study. (Numbers inside and outside the parenthesis are IoU on Pred View and GT View, respectively)} \\
\hline
RPS & {\color{black}SD} & car & sofa & airplane & bench & display & chair & table \\
\hline
 & & 0.747 (0.753) & 0.624 (0.643) & 0.557 (0.565) & 0.345 (0.460) & 0.457 (0.577) & 0.499 (0.508) & 0.406 (0.427) \\
 \hline
$\surd$ & & 0.782 (0.773) & 0.641 (0.639) & \textbf{0.644} (0.639) & 0.461 (0.485) & 0.597 (0.540) & 0.543 (0.538) & 0.512 (0.477) \\
\hline
$\surd$ & $\surd$ & \textbf{0.796} (\textbf{0.793}) & \textbf{0.651} (\textbf{0.649}) & \textbf{0.644} (\textbf{0.641}) & \textbf{0.500} (\textbf{0.500}) & \textbf{0.612} (\textbf{0.583}) & \textbf{0.544} (\textbf{0.541}) & \textbf{0.518} (\textbf{0.504}) \\
\hline
RPS & {\color{black}SD} & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
\hline
 & & 0.522 (\textbf{0.705}) & 0.597 (0.579) & 0.584 (0.614) & 0.574 (0.575) & 0.290 (0.421) & 0.500 (0.576) & 0.516 (0.569) \\
 \hline
$\surd$ & & 0.734 (0.673) & 0.696 (0.645) & 0.636 (0.599) & 0.585 (0.553) & \textbf{0.478} (\textbf{0.471}) & \textbf{0.619} (\textbf{0.627}) & 0.608 (0.588) \\
\hline
$\surd$ & $\surd$ & \textbf{0.738} (0.680) & \textbf{0.705} (\textbf{0.683}) & \textbf{0.651} (\textbf{0.623}) & \textbf{0.595} (\textbf{0.580}) & 0.469 (0.465) & \textbf{0.619} (0.619) & \textbf{0.618} (\textbf{0.604}) \\
\hline
\end{tabular}}
\end{center}

\label{table:tablevi}

\end{table*}

% %% table 4
% \begin{table*}[h]
% \begin{center}
% \caption{The sensitivity analysis for sampling different number of silhouettes}
% \scalebox{1}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{8}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow)$} \\
% \hline
%  & car & sofa & airplane & bench & display & chair & table \\
% \hline

% 2 Random Views (GT Pos)  & 0.795 & 0.641 & 0.642 & \textbf{0.502} & 0.610 & 0.538 & 0.494 \\
% 2 Random Views (Pred Pos) & 0.792 & 0.640 & 0.639 & \textbf{0.502} & 0.592 & 0.535 & 0.489 \\
% \hline
% 3 Random Views (GT Pos) & \textbf{0.796} & \textbf{0.651} &\textbf{0.644} & 0.500 & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} \\
% 3 Random Views (Pred Pos) & 0.793 & 0.649 & 0.641 & 0.500 & 0.583 & 0.541 & 0.504 \\
% \hline

%  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
% \hline
% 2 Random Views (GT Pos) & 0.723 & 0.697 & \textbf{0.658} & 0.586 & \textbf{0.470 }& \textbf{0.624} & 0.617 \\
% 2 Random Views (Pred Pos) & 0.675 & 0.676 & 0.638 & 0.582  & 0.465 & \textbf{0.624 }& 0.603 \\
% \hline
% 3 Random Views (GT Pos) & \textbf{0.738 }&\textbf{ 0.705} & 0.651 & \textbf{0.595 }& 0.469 & 0.619 &\textbf{0.618} \\ 
% 3 Random Views (Pred Pos) & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & 0.619 & 0.604 \\
% \hline
% \end{tabular}}
% \end{center}

% \label{table:tablevii}

% \end{table*}

% %% table 7
% \begin{table*}[h]
% \begin{center}
% \caption{The sensitivity analysis for sampling different number of silhouettes}
% \scalebox{1}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{8}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow)$} \\
% \hline
%  & car & sofa & airplane & bench & display & chair & table \\
% \hline

% 2 Random Views (GT Pos)  & 0.795 & 0.641 & 0.642 & \textbf{0.502} & 0.610 & 0.538 & 0.494 \\
% 2 Random Views (Pred Pos) & 0.792 & 0.640 & 0.639 & \textbf{0.502} & 0.592 & 0.535 & 0.489 \\
% \hline
% 3 Random Views (GT Pos) & \textbf{0.796} & \textbf{0.651} &\textbf{0.644} & 0.500 & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} \\
% 3 Random Views (Pred Pos) & 0.793 & 0.649 & 0.641 & 0.500 & 0.583 & 0.541 & 0.504 \\
% \hline

%  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
% \hline
% 2 Random Views (GT Pos) & 0.723 & 0.697 & \textbf{0.658} & 0.586 & \textbf{0.470 }& \textbf{0.624} & 0.617 \\
% 2 Random Views (Pred Pos) & 0.675 & 0.676 & 0.638 & 0.582  & 0.465 & \textbf{0.624 }& 0.603 \\
% \hline
% 3 Random Views (GT Pos) & \textbf{0.738 }&\textbf{ 0.705} & 0.651 & \textbf{0.595 }& 0.469 & 0.619 &\textbf{0.618} \\ 
% 3 Random Views (Pred Pos) & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & 0.619 & 0.604 \\
% \hline
% \end{tabular}}
% \end{center}

% \label{table:tablevii}

% \end{table*}


==> table/table4.tex <==
%% table 1
\begin{table*}[h]
\begin{center}
\caption{{The quantitative evaluation of sketch-view estimation}}
\scalebox{1}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{9}{|c|}{Shapenet-synthetic (MAE $\downarrow)$} \\
\hline
\multicolumn{2}{|c|}{}  & car & sofa & airplane & bench & display & chair & table \\
\hline
\multirow{2}{*}{Elevation} & Sketch2Model & 1.0751 & 1.5989 & 2.3899 & 1.8345 & 1.8944 & 1.8690 & 1.2857  \\
\cline{2-9} & \textbf{Ours} & \textbf{0.9029} & \textbf{1.395} & \textbf{2.2014} & \textbf{1.0168} & \textbf{1.6826} & \textbf{1.5422} & \textbf{1.0184} \\
\hline
\multirow{2}{*}{Azimuth} & Sketch2Model & 5.0986 & 11.0327 & 10.4171 & 43.7923 & 44.1861 & 8.6753 & \textbf{86.7654}  \\
\cline{2-9} & \textbf{Ours} & \textbf{4.3056} & \textbf{9.8532} & \textbf{9.7180} & \textbf{38.7755} & \textbf{43.2417} & \textbf{7.2630} & 87.6369 
 \\
\hline
%\end{tabular}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\multicolumn{2}{|c|}{} & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
\hline
\multirow{2}{*}{Elevation} & Sketch2Model & 2.2732 & 1.2148 & 2.4303 & 3.6884 & 4.4071 & 3.3226 & 2.2526 \\
\cline{2-9} & \textbf{Ours} & \textbf{2.0720} & \textbf{1.0168} & \textbf{2.0659} & \textbf{3.4014} & \textbf{4.0796} & \textbf{3.1199} & \textbf{1.9627} \\
\hline
\multirow{2}{*}{Azimuth} & Sketch2Model & 54.3659 & 41.7126 & 73.8672 & 34.5512 & \textbf{84.4146} & 11.2999 & 39.2445  \\
\cline{2-9} & \textbf{Ours} &  \textbf{51.2568} & \textbf{38.7755} & \textbf{72.6029} & \textbf{33.8180} & 84.7734 & \textbf{10.7342} & \textbf{37.9042} \\
\hline
\end{tabular}}
\end{center}

\label{table:table1}

\end{table*}

%% table 1
% \begin{table*}[h]
% \begin{center}
% \caption{{The quantitative evaluation of sketch-view estimation}}
% \scalebox{0.84}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{15}{|c|}{Shapenet-synthetic (MAE $\downarrow)$} \\
% \hline
% \multicolumn{2}{|c|}{}  & car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
% \hline
% \multirow{2}{*}{Elevation} & Sketch2Model & 1.0751 & 1.5989 & 2.3899 & 1.8345 & 1.8944 & 1.8690 & 1.2857 & 2.2732 & 1.2148 & 2.4303 & 3.6884 & 4.4071 & 3.3226 & 2.2526  \\
% \cline{2-9} & \textbf{Ours} & \textbf{0.9029} & \textbf{1.395} & \textbf{2.2014} & \textbf{1.0168} & \textbf{1.6826} & \textbf{1.5422} & \textbf{1.0184} & \textbf{2.072} & \textbf{1.0168} & \textbf{2.0659} & \textbf{3.4014} & \textbf{4.0796} & \textbf{3.1199} & \textbf{1.9627} \\
% \hline
% \multirow{2}{*}{Azimuth} & Sketch2Model & 5.0986 & 11.0327 & 10.4171 & 43.7923 & 44.1861 & 8.6753 & \textbf{86.7654} & 54.3659 & 41.7126 & 73.8672 & 34.5512 & \textbf{84.4146} & 11.2999 & 39.2445  \\
% \cline{2-9} & \textbf{Ours} & \textbf{4.3056} & \textbf{9.8532} & \textbf{9.7180} & \textbf{38.7755} & \textbf{43.2417} & \textbf{7.2630} & 87.6369  &  \textbf{51.2568} & \textbf{38.7755} & \textbf{72.6029} & \textbf{33.8180} & 84.7734 & \textbf{10.7342} & \textbf{37.9042}
%  \\
% \hline
% %\end{tabular}
% %\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
% \end{tabular}}
% \end{center}

% \label{table:table1}

% \end{table*}



==> table/table5.tex <==
% %% table 1
% \begin{table*}[ht]
% \begin{center}
% \caption{{{The quantitative evaluation of sketch-view estimation}}
% \scalebox{1}{

% \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

% \hline
% \multicolumn{15}{|c|}{Shapenet-synthetic (MAE $\downarrow)$} \\
% \hline
%  & car & sofa & airplane & bench & display & chair & table  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean\\
% \hline
% Sketch2Model & 1.0751 & 1.5989 & 2.3899 & 1.8345 & 1.8944 & 1.8690 & 1.2857 & 2.2732 & 1.2148 & 2.4303 & 3.6884 & 4.4071 & 3.3226 & 2.2526 \\
% Ours & 0.746 & 0.620 & 0.618 & 0.477 & 0.550 & 0.515 & 0.470 & 0.673 & 0.667 & 0.624 & 0.569 & 0.463 & 0.606 & 0.584 \\
% \hline
% \textbf{Ours (GT Pos)} & \textbf{0.796} & \textbf{0.651} & \textbf{0.644} & \textbf{0.500} & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} & \textbf{0.738} & \textbf{0.705} & \textbf{0.651} & \textbf{0.595} & \textbf{0.469} & \textbf{0.619} & \textbf{0.618} \\
% \textbf{Ours (Pred Pos)} & 0.793 & 0.649 & 0.641 & \textbf{0.500} & 0.583 & 0.541 & 0.504 & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & \textbf{0.619} & 0.604\\
% \hline
% \end{tabular}}
% \end{center}

% \label{table:table1}

% \end{table*}

%% table 1
\begin{table*}[ht]
\begin{center}
\caption{{{The quantitative evaluation of sketch-view estimation}}
\scalebox{1}{

\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}

\hline
\multicolumn{15}{|c|}{Shapenet-synthetic (MAE $\downarrow)$} \\
\hline
 & car & sofa & airplane & bench & display & chair & table  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean\\
\hline
Sketch2Model & 1.0751 & 1.5989 & 2.3899 & 1.8345 & 1.8944 & 1.8690 & 1.2857 & 2.2732 & 1.2148 & 2.4303 & 3.6884 & 4.4071 & 3.3226 & 2.2526 \\
Ours & 0.746 & 0.620 & 0.618 & 0.477 & 0.550 & 0.515 & 0.470 & 0.673 & 0.667 & 0.624 & 0.569 & 0.463 & 0.606 & 0.584 \\
\hline
\textbf{Ours (GT Pos)} & \textbf{0.796} & \textbf{0.651} & \textbf{0.644} & \textbf{0.500} & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} & \textbf{0.738} & \textbf{0.705} & \textbf{0.651} & \textbf{0.595} & \textbf{0.469} & \textbf{0.619} & \textbf{0.618} \\
\textbf{Ours (Pred Pos)} & 0.793 & 0.649 & 0.641 & \textbf{0.500} & 0.583 & 0.541 & 0.504 & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & \textbf{0.619} & 0.604\\
\hline
\end{tabular}}
\end{center}

\label{table:table1}

\end{table*}

==> table/table6.tex <==
% %% table 4
% \begin{table*}[t]
% \begin{center}
% \caption{The sensitivity analysis for sampling different number of silhouettes}
% \scalebox{1}{
% \begin{tabular}{|c|c|c|c|c|c|c|c|}
% \hline
% \multicolumn{8}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow)$} \\
% \hline
%  & car & sofa & airplane & bench & display & chair & table \\
% \hline

% 2 Random Views (GT Pos)  & 0.795 & 0.641 & 0.642 & \textbf{0.502} & 0.610 & 0.538 & 0.494 \\
% 2 Random Views (Pred Pos) & 0.792 & 0.640 & 0.639 & \textbf{0.502} & 0.592 & 0.535 & 0.489 \\
% \hline
% 3 Random Views (GT Pos) & \textbf{0.796} & \textbf{0.651} &\textbf{0.644} & 0.500 & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} \\
% 3 Random Views (Pred Pos) & 0.793 & 0.649 & 0.641 & 0.500 & 0.583 & 0.541 & 0.504 \\
% \hline

%  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
% \hline
% 2 Random Views (GT Pos) & 0.723 & 0.697 & \textbf{0.658} & 0.586 & \textbf{0.470 }& \textbf{0.624} & 0.617 \\
% 2 Random Views (Pred Pos) & 0.675 & 0.676 & 0.638 & 0.582  & 0.465 & \textbf{0.624 }& 0.603 \\
% \hline
% 3 Random Views (GT Pos) & \textbf{0.738 }&\textbf{ 0.705} & 0.651 & \textbf{0.595 }& 0.469 & 0.619 &\textbf{0.618} \\ 
% 3 Random Views (Pred Pos) & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & 0.619 & 0.604 \\
% \hline
% \end{tabular}}
% \end{center}

% \label{table:tablevii}

% \end{table*}


% table 4
\begin{table*}[h]
\begin{center}
\caption{The sensitivity analysis for sampling different number of silhouettes}
\scalebox{0.84}{
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{15}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow)$} \\
\hline
 & car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
\hline

2 Random Views (GT Pos)  & 0.795 & 0.641 & 0.642 & \textbf{0.502} & 0.610 & 0.538 & 0.494 & 0.723 & 0.697 & \textbf{0.658} & 0.586 & \textbf{0.470 }& \textbf{0.624} & 0.617 \\
2 Random Views (Pred Pos) & 0.792 & 0.640 & 0.639 & \textbf{0.502} & 0.592 & 0.535 & 0.489 & 0.675 & 0.676 & 0.638 & 0.582  & 0.465 & \textbf{0.624 }& 0.603 \\
\hline
3 Random Views (GT Pos) & \textbf{0.796} & \textbf{0.651} &\textbf{0.644} & 0.500 & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} & \textbf{0.738 }&\textbf{0.705} & 0.651 & \textbf{0.595 }& 0.469 & 0.619 &\textbf{0.618} \\
3 Random Views (Pred Pos) & 0.793 & 0.649 & 0.641 & 0.500 & 0.583 & 0.541 & 0.504  & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & 0.619 & 0.604 \\
\hline



\end{tabular}}
\end{center}

\label{table:tablevii}

\end{table*}



==> table/table7.tex <==
%% table 4
\begin{table*}[h]
\begin{center}
\caption{The sensitivity analysis for sampling different number of silhouettes}
\scalebox{1}{

\begin{tabular}{|c|c|ccccccc|}
\hline
\multicolumn{8}{|c|}{Shapenet-synthetic (Voxel IoU $\uparrow)$} \\

\hline
                partial level & method      & airplane       & bench          & cabinet        & car            & chair          & lamp           & rifle          \\ \hline
\multirow{2}{*}{0}  & sketch2model & 0.624          & 0.481          & \textbf{0.701} & 0.751          & 0.522          & \textbf{0.472} & 0.612          \\
                    & ours         & \textbf{0.632} & \textbf{0.510} & 0.692          & \textbf{0.782} & \textbf{0.526} & 0.467          & \textbf{0.631} \\ \hline
\multirow{2}{*}{10} & sketch2model & 0.560          & 0.454          & \textbf{0.675} & 0.695          & 0.483          & \textbf{0.445} & 0.565          \\
                    & ours         & \textbf{0.578} & \textbf{0.476} & 0.663          & \textbf{0.743} & \textbf{0.486} & 0.442          & \textbf{0.595} \\ \hline
\multirow{2}{*}{20} & sketch2model & 0.481          & 0.419          & \textbf{0.638} & 0.619          & \textbf{0.434} & \textbf{0.403} & 0.505          \\
                    & ours         & \textbf{0.506} & \textbf{0.438} & 0.635          & \textbf{0.689} & 0.432          & 0.402          & \textbf{0.543} \\ \hline
               partial level & method         & sofa           & table          & telephone      & watercraft     & diplay         & loudspeaker    & mean           \\ \hline
\multirow{2}{*}{0}  & sketch2model & 0.622          & 0.478          & 0.719          & \textbf{0.586} & \textbf{0.604} & \textbf{0.641} & 0.601          \\
                    & ours         & \textbf{0.640} & \textbf{0.510} & \textbf{0.758} & 0.584          & 0.589          & 0.631          & \textbf{0.611} \\ \hline
\multirow{2}{*}{10} & sketch2model & 0.580          & 0.437          & 0.704          & \textbf{0.549} & \textbf{0.573} & \textbf{0.628} & 0.565          \\
                    & ours         & \textbf{0.604} & \textbf{0.465} & \textbf{0.733} & 0.547          & 0.552          & 0.614          & \textbf{0.576} \\ \hline
\multirow{2}{*}{20} & sketch2model & 0.516          & 0.400          & 0.682          & 0.489          & \textbf{0.525} & \textbf{0.606} & 0.517          \\
                    & ours         & \textbf{0.550} & \textbf{0.425} & \textbf{0.711} & \textbf{0.499} & 0.499          & 0.595          & \textbf{0.532} \\ \hline
\end{tabular}}
\end{center}

\label{table:tablevii}

\end{table*}


==> table/table8.tex <==
\begin{table*}[!ht]
	\begin{center}
		\caption{Comparisons of mean Chamfer Distance on ShapeNet-Sketch dataset}
		\label{table:the Chamfer Distance}
		\scalebox{1}{
			\begin{tabular}{ccccccccccccc}
				\hline
				~ & car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp \\ 
				\hline
				Sketch2Model & 16.5391 & 35.1184 & 21.0765 & 24.6853 & 22.9207 & 66.5329 & 22.2305 & 18.8218 & 22.2107 & 23.035 & 17.4914 & 51.9116 \\
				Our & 15.2375 & 34.1573 & 21.1384 & 25.2345 & 20.8415 & 62.1423 & 21.1423 & 17.0235 & 22.8512 & 21.3546 & 16.2354 & 51.5675 \\
				\hline
		\end{tabular}}
	\end{center}
\end{table*}

==> table/table9.tex <==
\begin{table*}[!ht]
	\begin{center}
		\caption{{\color{red}The result for predicted camera pose}}
		\label{table:pose}
		\scalebox{0.9}{
			\begin{tabular}{ccccccccccccccc}
				\hline
				~ & car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\ 
				\hline
				Retrieval & 0.626 & 0.431 & 0.411 & 0.219 & 0.338 & 0.238 & 0.232 & 0.536 & 0.431 & 0.365 & 0.369 & 0.223 & 0.413 & 0.370 \\ 
				Auto-Encoder & 0.648 & \textbf{0.534} & 0.469 & 0.347 & 0.472 & 0.361 & 0.359 & 0.537 & 0.534 & \textbf{0.533} & 0.456 & 0.328 & 0.541 & 0.372 \\ 
				Sketch2Model(pred) & 0.649 & 0.528 & 0.479 & 0.357 & 0.435 & 0.383 & 0.361 & 0.551 & 0.547 & 0.526 & 0.450 & 0.336 & 0.510 & 0.470 \\
				Sketch2Model(gt) & 0.659 & \textbf{0.534} & 0.487 & 0.366 & 0.479 & 0.393 & 0.357 & \textbf{0.554} & \textbf{0.568} & 0.526 & 0.450 & \textbf{0.338} & 0.534 & 0.483 \\
				Ours(pred) & 0.686 & 0.531 & 0.495 & 0.376 & 0.473 & 0.405 & 0.369 & 0.513 & 0.554 & 0.519 & 0.453 & 0.330 & 0.548 & 0.481 \\ 
				Ours(gt) &\textbf{0.688} & 0.531 & \textbf{0.497} & \textbf{0.382} & \textbf{0.479} & \textbf{0.413} & \textbf{0.372} & 0.517 & 0.555 & 0.523 & \textbf{0.459} & 0.328 & \textbf{0.550} & \textbf{0.484} \\ 
				\hline
		\end{tabular}}
	\end{center}
\end{table*}

==> table_1/table1.tex <==
%% table 1
\begin{table*}[ht]
\begin{center}
\caption{The quantitative evaluation of ShapeNet-Synthetic dataset}
\scalebox{1}{
\begin{tabular}{c c c c c c c c}
\hline
\multicolumn{8}{c}{Shapenet-synthetic (Voxel Iou $\uparrow)$} \\
 & car & sofa & airplane & bench & display & chair & table \\
\hline
Retrieval & 0.667 & 0.483 & 0.513 & 0.38  & 0.385 & 0.346 & 0.311 \\

Auto-Encoder & 0.769 & 0.613 & 0.576 & 0.467 & 0.541 & 0.496 & 0.512 \\

Sketch2Model (GT Pos)  & 0.751 & 0.622 & 0.624 & 0.481 & 0.604 & 0.522 & 0.478 \\
Sketch2Model (Pred Pos) & 0.746 & 0.620 & 0.618 & 0.477 & 0.550 & 0.515 & 0.470 \\

\textbf{Ours (GT Pos)} & \textbf{0.796} & \textbf{0.651} & \textbf{0.644} & \textbf{0.500} & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} \\
\textbf{Ours (Pred Pos)} & 0.793 & 0.649 & 0.641 & \textbf{0.500} & 0.583 & 0.541 & 0.504 \\
\hline
 & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
\hline
Retrieval & 0.622 & 0.518 & 0.468 & 0.422 & 0.325 & 0.475 & 0.455 \\

Auto-Encoder & 0.706 & 0.663 & 0.629 & 0.556 & 0.431 & 0.605 & 0.582 \\

Sketch2Model (GT Pos) & 0.719 & 0.701 & 0.641 & 0.586 & 0.472 & 0.612 & 0.601 \\
Sketch2Model (Pred Pos) & 0.673 & 0.667 & 0.624 & 0.569 & 0.463 & 0.606 & 0.584 \\

\textbf{Ours (GT Pos)} & \textbf{0.738} & \textbf{0.705} & \textbf{0.651} & \textbf{0.595} & \textbf{0.469} & \textbf{0.619} & \textbf{0.618} \\ 
\textbf{Ours (Pred Pos)} & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & \textbf{0.619} & 0.604 \\
\hline
\end{tabular}}
\end{center}

\label{table:table2}

\end{table*}


==> table_1/table2.tex <==

%% table 2

\begin{table*}[ht]
\begin{center}
\caption{The quantitative evaluation of ShapeNet-Sketch dataset}
\scalebox{0.84}{

\begin{tabular}{c c c c c c c c c c c c c c c c}

\hline
\multicolumn{15}{c}{Shapenet-sketch (Voxel Iou $\uparrow$)} \\
 & car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean\\
\hline
Retrieval & 0.626 & 0.431 & 0.411 & 0.219 & 0.338 & 0.238 & 0.232 & 0.536 & 0.431 & 0.365 & 0.369 & 0.223 & 0.413 & 0.370\\

Auto-Encoder & 0.648 & 0.534 & 0.469 & 0.347 & 0.472 & 0.361 & 0.359 & 0.537 & 0.534 & 0.533 & 0.456 & 0.328 & 0.541 & 0.372 \\

Sketch2Model (GT Pos)  & 0.659 & 0.534 & 0.487 & 0.366 & 0.479 & 0.393 & 0.357 & 0.554 & \textbf{0.568} & 0.526 & 0.450 & \textbf{0.338} & 0.534 & 0.483 \\
Sketch2Model (Pred Pos) & 0.649 & 0.528 & 0.479 & 0.357 & 0.435 & 0.383 & 0.361 & 0.551 & 0.547 & 0.544 & 0.466 & 0.336 & 0.510 & 0.470\\

Sketch2Model + DA (GT Pos) & 0.679  & \textbf{0.548} & \textbf{0.526} & \textbf{0.367} & - & \textbf{0.398} & 0.357 & - & - & - & - & - & 0.535 & 0.489\\
Sketch2Model + DA (Pred Pos) & 0.659 & 0.533 & 0.515 & 0.362 & - & 0.385 & 0.360  & - & - & - & - & - & 0.511 & 0.475 \\

\textbf{Ours (GT Pos)} & 0.695 & 0.528 & 0.502 & 0.364 & \textbf{0.493} & 0.389 & 0.370 & \textbf{0.574} & 0.563 & \textbf{0.538} & \textbf{0.477} & 0.334 & 0.535 & 0.489 \\
\textbf{Ours (Pred Pos)} & 0.683 & 0.523 & 0.502 & 0.364 & 0.493 & 0.389 & \textbf{0.370} & 0.527 & 0.549 & 0.509 & 0.468 & 0.331 & 0.535 & 0.476 \\

\textbf{Ours + DA (GT Pos)}   & \textbf{0.699} & 0.538 & 0.517 & 0.362 & - & 0.390 & 0.360 & - & - & - & - & - & \textbf{0.545} & \textbf{0.491} \\
\textbf{Ours + DA (Pred Pos)} & 0.692 & 0.532 & 0.515 & 0.360 & - & 0.382 & 0.346  & - & - & - & - & - & \textbf{0.545} & 0.477\\
\hline

\end{tabular}}
\end{center}

\label{table:table3}

\end{table*}

==> table_1/table3.tex <==


%% table 3
\begin{table*}[hb]
\caption{{The quantitative evaluation of ablation study.} }
\begin{center}
\scalebox{1}{
\begin{tabular}{c c c c c c c c c }
\hline
\multicolumn{9}{c}{Ablation Study. (Numbers inside and outside the parenthesis are IoU on Pred View and GT View, respectively)} \\
\hline
RPS & SD & car & sofa & airplane & bench & display & chair & table \\
\hline
 & & 0.747 (0.753) & 0.624 (0.643) & 0.557 (0.565) & 0.345 (0.460) & 0.457 (0.577) & 0.499 (0.508) & 0.406 (0.427) \\
$\surd$ & & 0.782 (0.773) & 0.641 (0.639) & \textbf{0.644} (0.639) & 0.461 (0.485) & 0.597 (0.540) & 0.543 (0.538) & 0.512 (0.477) \\
$\surd$ & $\surd$ & \textbf{0.796} (\textbf{0.793}) & \textbf{0.651} (\textbf{0.649}) & \textbf{0.644} (\textbf{0.641}) & \textbf{0.500} (\textbf{0.500}) & \textbf{0.612} (\textbf{0.583}) & \textbf{0.544} (\textbf{0.541}) & \textbf{0.518} (\textbf{0.504}) \\
\hline
RPS & SD & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
\hline
 & & 0.522 (\textbf{0.705}) & 0.597 (0.579) & 0.584 (0.614) & 0.574 (0.575) & 0.290 (0.421) & 0.500 (0.576) & 0.516 (0.569) \\
$\surd$ & & 0.734 (0.673) & 0.696 (0.645) & 0.636 (0.599) & 0.585 (0.553) & \textbf{0.478} (\textbf{0.471}) & \textbf{0.619} (\textbf{0.627}) & 0.608 (0.588) \\
$\surd$ & $\surd$
 & \textbf{0.738} (0.680) & \textbf{0.705} (\textbf{0.683}) & \textbf{0.651} (\textbf{0.623}) & \textbf{0.595} (\textbf{0.580}) & 0.469 (0.465) & \textbf{0.619} (0.619) & \textbf{0.618} (\textbf{0.604}) \\
\hline
\end{tabular}}
\end{center}

\label{table:tablevi}

\end{table*}

==> table_1/table4.tex <==
%% table 1
\begin{table*}[ht]
\begin{center}
\caption{{The quantitative evaluation of sketch-view estimation}}
\scalebox{1}{
\begin{tabular}{c c c c c c c c c}
\hline
\multicolumn{9}{c}{Shapenet-synthetic (MAE $\downarrow)$} \\
 \hline
\multicolumn{2}{c}{}  & car & sofa & airplane & bench & display & chair & table \\
 \hline
\multirow{2}{*}{Elevation} & Sketch2Model & 1.0751 & 1.5989 & 2.3899 & 1.8345 & 1.8944 & 1.8690 & 1.2857  \\
 & \textbf{Ours} & \textbf{0.9029} & \textbf{1.395} & \textbf{2.2014} & \textbf{1.0168} & \textbf{1.6826} & \textbf{1.5422} & \textbf{1.0184} \\
 
\multirow{2}{*}{Azimuth} & Sketch2Model & 5.0986 & 11.0327 & 10.4171 & 43.7923 & 44.1861 & 8.6753 & \textbf{86.7654}  \\
 & \textbf{Ours} & \textbf{4.3056} & \textbf{9.8532} & \textbf{9.7180} & \textbf{38.7755} & \textbf{43.2417} & \textbf{7.2630} & 87.6369 
 \\
 
%\end{tabular}
%\begin{tabular}{|c|c|c|c|c|c|c|c|c|}
\hline
\multicolumn{2}{c}{} & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
\hline
\multirow{2}{*}{Elevation} & Sketch2Model & 2.2732 & 1.2148 & 2.4303 & 3.6884 & 4.4071 & 3.3226 & 2.2526 \\
 & \textbf{Ours} & \textbf{2.072} & \textbf{1.0168} & \textbf{2.0659} & \textbf{3.4014} & \textbf{4.0796} & \textbf{3.1199} & \textbf{1.9627} \\

\multirow{2}{*}{Azimuth} & Sketch2Model & 54.3659 & 41.7126 & 73.8672 & 34.5512 & \textbf{84.4146} & 11.2999 & 39.2445  \\
 & \textbf{Ours} &  \textbf{51.2568} & \textbf{38.7755} & \textbf{72.6029} & \textbf{33.8180} & 84.7734 & \textbf{10.7342} & \textbf{37.9042} \\
\hline
\end{tabular}}
\end{center}

\label{table:table1}

\end{table*}


==> table_1/table5.tex <==
%% table 1
\begin{table*}[ht]
\begin{center}
\caption{{{The quantitative evaluation of sketch-view estimation}}
\scalebox{1}{

\begin{tabular}{c c c c c c c c c c c c c c c c}

\hline
\multicolumn{15}{|c|}{Shapenet-synthetic (MAE $\downarrow)$} \\
\hline
 & car & sofa & airplane & bench & display & chair & table  & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean\\
\hline
Sketch2Model & 1.0751 & 1.5989 & 2.3899 & 1.8345 & 1.8944 & 1.8690 & 1.2857 & 2.2732 & 1.2148 & 2.4303 & 3.6884 & 4.4071 & 3.3226 & 2.2526 \\
Ours & 0.746 & 0.620 & 0.618 & 0.477 & 0.550 & 0.515 & 0.470 & 0.673 & 0.667 & 0.624 & 0.569 & 0.463 & 0.606 & 0.584 \\
\hline
\textbf{Ours (GT Pos)} & \textbf{0.796} & \textbf{0.651} & \textbf{0.644} & \textbf{0.500} & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} & \textbf{0.738} & \textbf{0.705} & \textbf{0.651} & \textbf{0.595} & \textbf{0.469} & \textbf{0.619} & \textbf{0.618} \\
\textbf{Ours (Pred Pos)} & 0.793 & 0.649 & 0.641 & \textbf{0.500} & 0.583 & 0.541 & 0.504 & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & \textbf{0.619} & 0.604\\
\hline
\end{tabular}}
\end{center}

\label{table:table1}

\end{table*}


==> table_1/table6.tex <==
%% table 4
\begin{table*}[h]
\begin{center}
\caption{The sensitivity analysis for sampling different number of silhouettes}
\scalebox{1}{
\begin{tabular}{c c c c c c c c}
\hline
\multicolumn{8}{c}{Shapenet-synthetic (Voxel Iou $\uparrow)$} \\
\hline
 & car & sofa & airplane & bench & display & chair & table \\
\hline

2 Random Views (GT Pos)  & 0.795 & 0.641 & 0.642 & \textbf{0.502} & 0.610 & 0.538 & 0.494 \\
2 Random Views (Pred Pos) & 0.792 & 0.640 & 0.639 & \textbf{0.502} & 0.592 & 0.535 & 0.489 \\

3 Random Views (GT Pos) & \textbf{0.796} & \textbf{0.651} &\textbf{0.644} & 0.500 & \textbf{0.612}	& \textbf{0.544} & \textbf{0.518} \\
3 Random Views (Pred Pos) & 0.793 & 0.649 & 0.641 & 0.500 & 0.583 & 0.541 & 0.504 \\
\hline

 & telephone & cabinet & loudspeaker & watercraft & lamp & rifile & mean \\
\hline
2 Random Views (GT Pos) & 0.723 & 0.697 & \textbf{0.658} & 0.586 & \textbf{0.470 }& \textbf{0.624} & 0.617 \\
2 Random Views (Pred Pos) & 0.675 & 0.676 & 0.638 & 0.582  & 0.465 & \textbf{0.624 }& 0.603 \\

3 Random Views (GT Pos) & \textbf{0.738 }&\textbf{ 0.705} & 0.651 & \textbf{0.595 }& 0.469 & 0.619 &\textbf{0.618} \\ 
3 Random Views (Pred Pos) & 0.680 & 0.683 & 0.623 & 0.580 & 0.465 & 0.619 & 0.604 \\
\hline
\end{tabular}}
\end{center}

\label{table:tablevii}

\end{table*}


==> table_1/table7.tex <==
%% table 4
\begin{table*}[h]
\begin{center}
\caption{The sensitivity analysis for sampling different number of silhouettes}
\scalebox{1}{

\begin{tabular}{|c|c|ccccccc|}
\hline
\multicolumn{8}{|c|}{Shapenet-synthetic (Voxel Iou $\uparrow)$} \\

\hline
                partial level & method      & airplane       & bench          & cabinet        & car            & chair          & lamp           & rifle          \\ \hline
\multirow{2}{*}{0}  & sketch2model & 0.624          & 0.481          & \textbf{0.701} & 0.751          & 0.522          & \textbf{0.472} & 0.612          \\
                    & ours         & \textbf{0.632} & \textbf{0.510} & 0.692          & \textbf{0.782} & \textbf{0.526} & 0.467          & \textbf{0.631} \\ \hline
\multirow{2}{*}{10} & sketch2model & 0.560          & 0.454          & \textbf{0.675} & 0.695          & 0.483          & \textbf{0.445} & 0.565          \\
                    & ours         & \textbf{0.578} & \textbf{0.476} & 0.663          & \textbf{0.743} & \textbf{0.486} & 0.442          & \textbf{0.595} \\ \hline
\multirow{2}{*}{20} & sketch2model & 0.481          & 0.419          & \textbf{0.638} & 0.619          & \textbf{0.434} & \textbf{0.403} & 0.505          \\
                    & ours         & \textbf{0.506} & \textbf{0.438} & 0.635          & \textbf{0.689} & 0.432          & 0.402          & \textbf{0.543} \\ \hline
               partial level & method         & sofa           & table          & telephone      & watercraft     & diplay         & loudspeaker    & mean           \\ \hline
\multirow{2}{*}{0}  & sketch2model & 0.622          & 0.478          & 0.719          & \textbf{0.586} & \textbf{0.604} & \textbf{0.641} & 0.601          \\
                    & ours         & \textbf{0.640} & \textbf{0.510} & \textbf{0.758} & 0.584          & 0.589          & 0.631          & \textbf{0.611} \\ \hline
\multirow{2}{*}{10} & sketch2model & 0.580          & 0.437          & 0.704          & \textbf{0.549} & \textbf{0.573} & \textbf{0.628} & 0.565          \\
                    & ours         & \textbf{0.604} & \textbf{0.465} & \textbf{0.733} & 0.547          & 0.552          & 0.614          & \textbf{0.576} \\ \hline
\multirow{2}{*}{20} & sketch2model & 0.516          & 0.400          & 0.682          & 0.489          & \textbf{0.525} & \textbf{0.606} & 0.517          \\
                    & ours         & \textbf{0.550} & \textbf{0.425} & \textbf{0.711} & \textbf{0.499} & 0.499          & 0.595          & \textbf{0.532} \\ \hline
\end{tabular}}
\end{center}

\label{table:tablevii}

\end{table*}


==> table_new/Sketch_cd.tex <==
\begin{table*}[!ht]
	\begin{center}
		\caption{Comparisons of mean Chamfer Distance on ShapeNet-Sketch dataset}
		\label{table:Sketch cd}
		\scalebox{0.85}{
			\renewcommand{\arraystretch}{1.5}
			\begin{tabular}{lcccccccccccccc}
				\hline
                \multicolumn{15}{c}{Shapenet-Sketch (Chamfer Distance $\downarrow)$} \\
				~ & car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp & rifle & mean\\ 
				\hline
				Sketch2Model & 16.5391 & 35.1184 & \textbf{21.0765} & \textbf{24.6853} & 22.9207 & 66.5329 & 22.2305 & 18.8218 & \textbf{22.2107} & 23.0350 & 17.4914 & 51.9116 & 21.2319 & 27.9850 \\
				Our & \textbf{15.2375} & \textbf{34.1573} & 21.1384 & 25.2345 & \textbf{20.8415} & \textbf{62.1423} & \textbf{21.1673} & \textbf{17.0235} & 22.8512 & \textbf{21.3546} & \textbf{16.2354} & \textbf{51.5675} & \textbf{20.7533} &  \textbf{26.9003}\\
				\hline
		\end{tabular}}
	\end{center}
\end{table*}

==> table_new/Sketch_iou.tex <==
\begin{table*}[ht]
	\begin{center}
            
		
		\label{table:Sketch iou}
            \setlength{\tabcolsep}{2.5mm}{
		\resizebox{\textwidth}{!}{
			
			\begin{tabular}{lllllllllllllll}
				
				\hline
				\multicolumn{15}{c}{Shapenet-sketch (Voxel IoU $\uparrow$)} \\
				& car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp & rifle & mean\\
				\hline
				Retrieval & 0.626 & 0.431 & 0.411 & 0.219 & 0.338 & 0.238 & 0.232 & 0.536 & 0.431 & 0.365 & 0.369 & 0.223 & 0.413 & 0.370\\
				Auto-Encoder & 0.648 & \textbf{0.534} & 0.469 & 0.347 & 0.472 & 0.361 & 0.359 & 0.537 & 0.534 & \textbf{0.533} & 0.456 & 0.328 & 0.541 & 0.372 \\
%				Sketch2Model  & 0.659 & \textbf{0.534} & 0.487 & 0.366 & 0.479 & 0.393 & 0.357 & \textbf{0.554} & \textbf{0.568} & 0.526 & 0.450 & \textbf{0.338} & 0.534 & 0.483 \\
				\textbf{Ours} & \textbf{0.688} & 0.531 & \textbf{0.497} & \textbf{0.382} & \textbf{0.479} & \textbf{0.413} & \textbf{0.372} & 0.517 & 0.555 & 0.523 & \textbf{0.459} & 0.328 & \textbf{0.550} & \textbf{0.484} \\
				\hline
				
		\end{tabular}}}
  \caption{The Voxel IoU of ShapeNet-Sketch dataset}
	\end{center}
\end{table*}

==> table_new/Synthetic_cd.tex <==
\begin{table*}[b]
	\begin{center}
		\caption{Comparisons of mean Chamfer Distance on ShapeNet-Synthetic dataset}
		\label{table:Synthetic cd}
		\scalebox{0.85}{
			\renewcommand{\arraystretch}{1.5}
			\begin{tabular}{lcccccccccccccc}
				\hline
				\multicolumn{15}{c}{Shapenet-Synthetic (Chamfer Distance $\downarrow)$} \\
				& car & sofa & airplane & bench & display & chair & table & telephone & cabinet & loudspeaker & watercraft & lamp & rifle & mean \\
				\hline
				Sketch2Model & 15.2595 & \textbf{42.3509} & 22.9386 & 23.3147 & \textbf{24.0722} & 61.9558 & \textbf{21.8722} & 18.8203 & \textbf{18.6660} & \textbf{20.7303} & 15.7249 & 60.3407 & 19.0046 & 28.0808 \\
				Ours & \textbf{14.3651} & 47.1434 & \textbf{22.1654} & \textbf{23.0716} & 25.0740 & \textbf{27.8526} & 22.9202 & \textbf{18.0563} & 23.3107 & 23.4705 & \textbf{15.0412} & \textbf{51.2210} & \textbf{18.1983} & \textbf{25.5300} \\
			
				\hline
		\end{tabular}}
	\end{center}
	
\end{table*}
